Functional Geometry Guided Protein Sequence and Backbone Structure Co-Design

Proteins are macromolecules responsible for essential functions in almost all living organisms. Designing reasonable proteins with desired functions is crucial. A protein's sequence and structure are strongly correlated and they together determine its function. In this paper, we propose NAEPro, a model to jointly design Protein sequence and structure based on automatically detected functional sites. NAEPro is powered by an interleaving network of attention and equivariant layers, which can capture global correlation in a whole sequence and local influence from nearest amino acids in three dimensional (3D) space. Such an architecture facilitates effective yet economic message passing at two levels. We evaluate our model and several strong baselines on two protein datasets, $\beta$-lactamase and myoglobin. Experimental results show that our model consistently achieves the highest amino acid recovery rate, TM-score, and the lowest RMSD among all competitors. These findings prove the capability of our model to design protein sequences and structures that closely resemble their natural counterparts. Furthermore, in-depth analysis further confirms our model's ability to generate highly effective proteins capable of binding to their target metallocofactors. We provide code, data and models in Github.

==> 002background.tex <==
\subsection{Equivariance and Invariance}
\textbf{Equivariant Function}
A function $f$ is said to be equivariant to the action of a group $\mathcal{G}$ if $T_g(f(x))$ = $f(S_g(x))$ for all $g \in \mathcal{G}$, where $S_g$, $T_g$ are linear representations related to the group element~\citep{serre1977linear}. 
In this work, we consider the Euclidean group $E(3)$ generated by translations, rotations and reflections, for which $S_g$ and $T_g$ can be represented by a translation $t$ and an orthogonal matrix $R$ that rotates or reflects coordinates. $f$ is then equivariant to a translation $t$, rotation or reflection $R$ if transforming its input results in an equivalent transformation of its output, i.e. $f(Rx+t)=Rf(x)+t$.

\textbf{Invariant Distribution}
In our setting, a conditional distribution $p(y|x)$ is invariant to the action of rotation or reflection $R$ when:
\begin{equation}
\small 
p(y|x)=p(Ry|Rx)\; \text{or} \; p(y|x)=p(y|Rx)\qquad  \text{for all orthogonal matrix $R$} 
\end{equation}
% A conditional distribution is also invariant to $R$ transformations if:
% \begin{equation}
% \small 
% p(y|x)=p(y|Rx)\qquad  \text{for all orthogonal matrix $R$} 
% \end{equation} 
% \citet{xu2022geodiff} proved that if x $\sim$ p(x) is invariant to a group and the transition probabilities of a Markov chain y $\sim$ p(y|x) are equivariant, then the marginal distribution of y is invariant to group transformations as well.

\subsection{E(n) Equivariant Graph Neural Networks (EGNNs)}
EGNNs~\citep{satorras2021n} are a type of Graph Neural Network that satisfies the equivariance constraint. In this work, we consider interactions between all C$_\alpha$ in the backbone structure, and therefore assume a fully connected graph $\mathcal{G}$ with nodes $v_i \in V$.
Each node $v_i$ is endowed with coordinates $x_i \in R^3$ as well as $d$-dimensional features $h_i \in R^d$. In this setting, EGNN consists of the composition of equivariant convolutional layers~(EGCL): $x^{(l+1)},h^{(l+1)} = \text{EGCL}[x^l, h^l]$, which are defined as:
\begin{equation}
\begin{split}
\small 
m_{ij}&=\phi_e(h_i^l, h_j^l, d_{ij}^2, a_{ij}), \quad h_i^{l+1} = \phi_h(h_i^l, \sum_{j\ne i}\Tilde{e}_{ij}m_{ij}) \\
x_i^{l+1} &= x_i^l + \sum_{j\ne i}\frac{x_i^l-x_j^l}{d_{ij}+1}\phi_x(h_i^l, h_j^l, d_{ij}^2, a_{ij})
\end{split}
\label{equation_egnn}
\end{equation}
where $l$ indexes the layer, and $d_{ij} = ||x_i^l-x^l_j||_2$ is the Euclidean distance between nodes $(v_i, v_j)$, and $a_{ij}$ are optional edge attributes. 
$\Tilde{e}_{ij}=\phi_{inf}(m_{ij})$ is the attention score. 
All learnable components $(\phi_e,\phi_h,\phi_x,\phi_{inf})$ are parametrized by fully connected neural networks.
An entire EGNN architecture is then composed of $L$ EGCL layers, which applies the following non-linear transformation: $\hat{x}, \hat{h} = \text{EGNN}[x^0, h^0]$. This transformation satisfies the required equivariant property:
\begin{equation}
\small 
R\hat{x} + t, \hat{h} = \text{EGNN}[Rx^0 + t, h^0]\qquad   \text{for all orthogonal matrix $R$ and $t\in R^3$}
\label{equation:EGNNs}
\end{equation}
